Application-Level Validation of Accelerator Designs Using a Formal Software/Hardware Interface

Ideally, accelerator development should be as easy as software development. Several recent design languages/tools are working toward this goal, but actually testing early designs on real applications end-to-end remains prohibitively difficult due to the costs of building specialized compiler and simulator support. We propose a new first-in-class, mostly automated methodology termed "3LA" to enable end-to-end testing of prototype accelerator designs on unmodified source applications. A key contribution of 3LA is the use of a formal software/hardware interface that specifies an accelerator's operations and their semantics. Specifically, we leverage the Instruction-Level Abstraction (ILA) formal specification for accelerators that has been successfully used thus far for accelerator implementation verification. We show how the ILA for accelerators serves as a software/hardware interface, similar to the Instruction Set Architecture (ISA) for processors, that can be used for automated development of compilers and instruction-level simulators. Another key contribution of this work is to show how ILA-based accelerator semantics enables extending recent work on equality saturation to auto-generate basic compiler support for prototype accelerators in a technique we term "flexible matching." By combining flexible matching with simulators auto-generated from ILA specifications, our approach enables end-to-end evaluation with modest engineering effort. We detail several case studies of 3LA, which uncovered an unknown flaw in a recently published accelerator and facilitated its fix.

==> Customizations/lst_style_verilog.tex <==
\lstdefinestyle{verilog-style}
{
  language=Verilog,
  basicstyle=\small\ttfamily,
  % numbers=none,
  frame=l,
  moredelim=*[s][\colorIndex]{[}{]},
  literate=*{:}{:}1
}

\definecolor{vorange}{RGB}{255,143,102}

\makeatletter
\newcommand*\@lbracket{[}
\newcommand*\@rbracket{]}
\newcommand*\@colon{:}
\newcommand*\colorIndex{%
  \edef\@temp{\the\lst@token}%
  \ifx\@temp\@lbracket \color{black}%
  \else\ifx\@temp\@rbracket \color{black}%
  \else\ifx\@temp\@colon \color{black}%
  \else \color{vorange}%
  \fi\fi\fi
}
\makeatother

==> Floats/lst-concrete-mapping.tex <==
\begin{figure*}[!tb]
\begin{lstlisting}[language=c]
%1 = nn.dense(%input, %weight)
%4 = nn.bias_add(%1, %bias)
\end{lstlisting}
(a) Compiler IR instructions

\begin{lstlisting}[language=c]
ComILA.relay_nn_dense           %out %input %weight
ComILA.relay_bias_add           %out %in_0 %in_1
\end{lstlisting}
(b) Compiler IR ILA program fragment\\

\begin{lstlisting}[language=c]
// 1. writing data into the accelerator memory
FlexASR_ILA.write_v                  %addr %data
...
// 2. configuring the accelerator for executing linear layer operation
FlexASR_ILA.pe_cfg_rnn_layer_sizing %pe_idx %is_zero %is_cluster %is_bias %num_mngr %num_v_out
FlexASR_ILA.pe_cfg_mngr %pe_idx %mngr_idx %is_zero %bias_w %bias_b %bias_i %num_v_in %base_w\
                        %base_b %base_i
FlexASR_ILA.pe_cfg_act_mngr %pe_idx %is_zero %bias %num_insn %num_v_out %buf_base %out_base
FlexASR_ILA.pe_cfg_act_v %pe_idx %is_zero %insn_0 %insn_1
FlexASR_ILA.gb_cfg_mmngr_gb_large %base_0 %num_v_0 %base_1 %num_v_1
FlexASR_ILA.gb_cfg_gb_control %mode %is_rnn %mem_id_in %mem_id_out %num_v_in %num_v_out %num_ts
// 3. triggering the accelerator linear function 
FlexASR_ILA.fn_start                 %fn_id
// 4. reading data out from the accelerator memory (if needed)
FlexASR_ILA.read_v                   %addr
...
\end{lstlisting}
(c) FlexASR ILA program fragment\\

\begin{lstlisting}[language=c]
// 1. writing data into the accelerator memory
Write, addr=0xA4500000, data=0x0F0EFFBF8F746F9FB58D148E0EB7BFDAD
...
// 2. configurating the accelerator states for linear layer operation
Write, addr=0xA4400010, data=0x0010101000001
Write, addr=0xA4400020, data=0x0000000010000000102020200
Write, addr=0xA4800010, data=0x0000000000102050001
...
// 3. triggering the accelerator function
Write, addr=0xA3000010, data=0x1
// 4. reading data out from the accelerator memory (if needed)
Read,  addr=0xA3500200, data=0x0
...
\end{lstlisting}
(d) FlexASR MMIO commands

\caption{\textbf{IR-accelerator mapping for the FlexASR LinearLayer operation.}
This shows a many-to-many mapping from Relay IR instrucions to a sequence of FlexASR MMIO commands.
(a) LinearLayer in Relay consists of a linear transformation operation \texttt{\small nn.dense}, followed by a bias addition operation \texttt{\small nn.bias\_add}.
(b) The compiler IR ILA instruction has an one-to-one mapping to the compiler IR instruction. 
(c) The FlexASR ILA program fragment in its assembly format: It includes: (1) write instructions to transfer the data into FlexASR's memory. (2) setting up FlexASR \texttt{LinearLayer} configuration states, for example, the instruction at line 5 sets the states of FlexASR layer sizing information. (3) instruction that triggers the FlexASR \texttt{LinearLayer} computation (5) read data out from FlexASR's memory if needed.
(d) The MMIO commands for FlexASR have a one-to-one mapping to its FlexASR ILA instructions.
}
\label{fig.concrete-mapping}
\Description[]{}
\end{figure*}


==> Floats/lst-maxpool.tex <==

\begin{lstlisting}[language=lisp]
; (a) IR-accelerator rewrite rule for FlexASR's temporal max-pooling (which corresponds to 
; 2D max-pooling with window shape and stride (2, 1))
(map reduceMax (windows (2, 1) (2, 1) ?T)) -> (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore ?T)))

; (b) Initial Glenside program for a 2D max-pooling layer with window shape (4, 4) 
; and stride (2, 2). We use T to denote the input of the 2D max-pooling layer.
(map reduceMax (windows (4, 4) (2, 2) T))

; (c) A rewritten IR program found via Glenside
; T denotes the input of the 2D max-pooling layer 
; S is the shape of the output of the 2D max-pooling layer
(reshape (map reduceMax (windows (2, 1) (2, 1) 
         (map reduceMax (windows (2, 1) (2, 1) 
         (map reduceMax (windows (2, 1) (2, 1) 
         (map reduceMax (windows (2, 1) (2, 1) 
            (map flatten (windows (4, 4) (2, 2) T)) )))))))) S)

; (d) 2D max-pooling using FlexASR
(reshape (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore 
         (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore 
         (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore 
         (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore 
            (map flatten (windows (4, 4) (2, 2) T)) )))))))))))) S)

; (e) IR-accelerator rewrite rule to remove redundant Store-Loads
; Loading data out of the accelerator only to store it back to the same location is unnecessary
(fasrMaxpStore (fasrMaxpLoad ?T) -> ?T

; (f) Optimized 2D max-pooling using FlexASR
(reshape (fasrMaxpLoad (fasrMaxpool (fasrMaxpool (fasrMaxpool (fasrMaxpool (fasrMaxpStore 
    (map flatten (windows (4, 4) (2, 2) T)) )))))) S)
\end{lstlisting}

% \begin{subfigure}{\textwidth}
%     \begin{lstlisting}
% (map reduceMax (windows (4, 4) (2, 2) T))
%     \end{lstlisting}
%     % \begin{align*}
%     %     &\texttt{(map reduceMax (windows (4, 4) (2, 2) $T$))}
%     % \end{align*}
%     \caption{Initial Glenside program for a 2D max-pooling layer,
%     where $T$ is the output of the previous layer.}
%     \label{fig.maxpool.proginit}
% \end{subfigure}

% \begin{subfigure}{\textwidth}
%     \begin{lstlisting}
% (map reduceMax (windows (2, 1) (2, 1) ?T)) -> (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore ?T)))
%     if ?T has shape (m, n) where m % 2 == 0, n % 16 == 0
%     \end{lstlisting}
%     \small
%     % \begin{align*}
%     %     &\texttt{(map reduceMax (windows (2, 1) (2, 1) ?T))} \rightarrow \\
%     %     &\quad\texttt{(fasrMaxpLoad (fasrMaxpool (fasrMaxpStore ?T)))} \\
%     %     &\quad\texttt{if ?T has shape $(m, n)$ where $m$ \% 2 == 0, $n$ \% 16 == 0}
%     % \end{align*}
%     \caption{IR-accelerator rewrite rule for FlexASR's temporal max-pooling}
%     \label{fig.maxpool.rewriterule}
% \end{subfigure}

% \begin{subfigure}{\textwidth}
%     \begin{lstlisting}
% (reshape (map reduceMax (windows (2, 1) (2, 1) (map reduceMax (windows (2, 1) (2, 1) (map reduceMax (windows (2, 1) (2, 1) 
%   (map reduceMax (windows (2, 1) (2, 1) (map flatten (windows (4, 4) (2, 2) T)) )))))) (64, 64))
%     \end{lstlisting}
%     % \small
%     % \begin{align*}
%     %     &\texttt{(reshape (map reduceMax (windows (2, 1) (2, 1)} \\
%     %     &\quad \texttt{(map reduceMax (windows (2, 1) (2, 1)} \\
%     %     &\qquad \texttt{(map reduceMax (windows (2, 1) (2, 1)} \\
%     %     &\qquad\quad \texttt{(map reduceMax (windows (2, 1) (2, 1)} \\
%     %     &\qquad\quad \texttt{
%     %         (map flatten (windows (4, 4) (2, 2) $T$))
%     %     } \\
%     %     &\texttt{)))))) (64, 64))}
%     % \end{align*}
%     \caption{An implementation of the 2D max-pooling layer found during flexible-matching}
%     \label{fig.maxpool.progfound}
% \end{subfigure}

% \begin{subfigure}{\textwidth}
%     \begin{lstlisting}
% (reshape (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore (fasrMaxpLoad (fasrMaxpool 
%     (fasrMaxpStore (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore (map flatten (windows (4, 4) (2, 2) T)) )))))))))))) (64, 64))
%     \end{lstlisting}
%     % \small
%     % \begin{align*}
%     %     &\texttt{(reshape (fasrMaxpLoad (fasrMaxpool (fasrMaxpStore} \\
%     %     &\quad \texttt{(fasrMaxpLoad (fasrMaxpool (fasrMaxpStore} \\
%     %     &\qquad \texttt{(fasrMaxpLoad (fasrMaxpool (fasrMaxpStore} \\
%     %     &\qquad\quad \texttt{(fasrMaxpLoad (fasrMaxpool (fasrMaxpStore} \\
%     %     &\qquad\quad \texttt{
%     %         (map flatten (windows (4, 4) (2, 2) $T$))
%     %     } \\
%     %     &\texttt{)))))))))))) (64, 64))}
%     % \end{align*}
%     \caption{2D max-pooling using FlexASR}
%     \label{fig.maxpool.progaccel}
% \end{subfigure}

% \begin{subfigure}{\textwidth}
%     \begin{lstlisting}
% (reshape (fasrMaxpLoad (fasrMaxpool (fasrMaxpool (fasrMaxpool (fasrMaxpool (fasrMaxpStore 
%     (map flatten (windows (4, 4) (2, 2) T)) )))))) (64, 64))
%     \end{lstlisting}
%     % \small
%     % \begin{align*}
%     %     &\texttt{(reshape (fasrMaxpLoad} \\
%     %     &\quad \texttt{(fasrMaxpool (fasrMaxpool (fasrMaxpool (fasrMaxpool } \\
%     %     &\quad \texttt{
%     %         (fasrMaxpStore (map flatten (windows (4, 4) (2, 2) $T$))
%     %     } \\
%     %     &\texttt{)))))) (64, 64))}
%     % \end{align*}
%     \caption{Optimized 2D max-pooling using FlexASR}
%     \label{fig.maxpool.progopt}
% \end{subfigure}

% \hl{Akash: renamed compute to map, moved shape and stride arguments to start of windows rather than end.}


